Adapting Persistent Data Structures for Concurrency and Speculation

This work unifies insights from the systems and functional programming communities, in order to enable compositional reasoning about software which is nonetheless efficiently realizable in hardware. It exploits a correspondence between design goals for efficient concurrent data structures and efficient immutable persistent data structures, to produce novel implementations of mutable concurrent trees with low contention and an efficient snapshot operation to support speculative execution models. It also exploits commutativity to characterize a design space for integrating traditional high-performance concurrent data structures into Software Transactional Memory (STM) runtimes, and extends this technique to yield a novel algorithm for concurrent execution of so-called ``smart contracts'' (specialized programs which manipulate the state of blockchain ledgers).

==> proust/opacityopt.tex <==
\newcommand\anno[1]{$\langle\!\!\langle$#1$\rangle\!\!\rangle$}

\paragraph{Optimistic synchronization with eager updates.} 
We now turn to the question of opacity in the context
of optimistic synchronization, with
both conflict abstractions as well as
shadow copies.
Recall that a conflict detected in \var{mem}[$\alpha,\beta,...$]
means that two Proustian object operations do not commute.
In what follows, we annotate the elements of the algorithm with
their corresponding Push/Pull rule using the notation \anno{...}.

As shown in Figure~\ref{fig:designspaces}, the key requirement for
this version is that the
underlying STM detects (read/write \emph{and} write/write) conflicts
eagerly.



\begin{theorem}\label{thm:opteager} Eager/Optimistic Proust is opaque if the underlying STM detects all conflicts eagerly.
  \begin{proof}(Sketch)
For non-commutative operations $m_i$ and $n_j$ from
different uncommitted transactions, there will be some memory location
$\gamma \in CA(m_i) \cap CA(n_j)$ (Definition~\ref{def:ca}).
WLOG, $m$ performs a \var{write} to $\alpha^1_i,\alpha^2_i,\dots\in CA(m_i)$
before performing operation $m_i$, and $n$ either \var{read}s or \var{write}s  to $\alpha^1_j,\alpha^2_j,\dots\in CA(n_j)$
Therefore, $m$ and $n$ will perform conflicting operations on \var{mem}[$\gamma$], and at least one will aborted.
Aborted transaction perform their recorded inverse operations and---following the same argument used for boosting~\cite{HerlihyK2008,KP:PLDI2015}---the
commutative nature of the operations performed thus far ensures that
the inverses will not be visible to concurrent transactions.


Given the definition of conflict abstraction  (Definition~\ref{def:ca}),
if there are non-commutative operations $m_i$ and $n_j$ from
different uncommitted transactions, there will be some memory location
$\gamma \in CA(m_i) \cap CA(n_j)$.
In our eager implementation a transaction first performs a \var{write}
operation on memory locations $\alpha^1_i,\alpha^2_i,\dots\in CA(m_i)$
before performing operation $m_i$
\anno{ \APPLY{}($m_i$) and try to \PUSH{}($m_i$) }.
Therefore, both transactions will attempt
to write \var{mem}[$\gamma$]. Due to the eager nature,
this \var{mem}[$\gamma$] conflict will be detected and the second of the two 
transactions will be aborted before it performs its Proustian operation
\anno{ failing to \PUSH{}($m_i$) }.
The aborted transaction will perform inverse operations
\anno{ invoking \PUSH{}($m_{i-1}$);\UNAPP{}($m_{i-1}$), etc in reverse order}
and---following the same argument used for boosting~\cite{HerlihyK2008,KP:PLDI2015}---the
commutative nature of the operations performed thus far ensures that
the inverses will not be visible to concurrent transactions.
If a transaction commits,
the underlying STM will ensure that
writes to both regions of \var{mem} will become permanent,
with no effect on concurrent transactions whose reads/writes to \var{mem} are
treated with eager conflict detection \anno{ \CMT{} }.
Since this variant operates directly on the Proustian objects,
the committed effects are immediately visible \anno{ other transactions
  \PULL{} all before each subsequent \APPLY{} }.

  \end{proof}
\end{theorem}

\paragraph{Optimistic synchronization with lazy updates.} 
This variant is designed to exploit an STM that performs \emph{lazy}
read/write and lazy write/write conflict detection
(Figure~\ref{fig:designspaces}).  In these circumstances, since
conflict is detected late in the game (at commit time), it would be
dangerous to allow uncommitted transactions to perform mutation
operations directly on the shared state.

In response, shadow copy data structures
(Section~\ref{section:shadow}) allow transactions to proceed with
operations on Proustian objects (and observe their corresponding
return values) without exposing these effects to concurrent
uncommitted transactions. Shadow copies permit active transactions to
logically ``clone'' their own replica of the current committed
version, but it is not a full ``clone'' because the shadow copy may
rely on the latest committed version to generate return values.
To mitigate this, we surround execution of a Proustian operation $m_i$
with the relevant conflict abstraction operations $CA(m_i)$ as:
\[\begin{array}{l}
\textsf{foreach } \alpha \in CA(m_i) \textsf{ do write}(\alpha) \textsf{ done;}\\
m_i(); \\
\textsf{foreach } \alpha \in CA(m_i) \textsf{ do read}(\alpha) \textsf{ done;}\\
\end{array}\]
By pairing \var{write} and \var{read} operations on either side of the data structure access, we first announce the intention to write, thus forestalling an opacity violation due to write/write conflict, and then revalidate that access against any commits which may have taken place concurrently with the access, thus forestalling an opacity violation due to read/write conflict.



\begin{theorem}\label{thm:optlazy} Lazy/Optimistic Proust is opaque.
  \begin{proof}(Sketch)
Shadow copies permit active transactions to ``clone'' their
own replica of the current committed version (using a couple of
different implementation strategies) \anno{\PULL{}($n$) for only committed $n$}.
It is not a full ``clone'' because the shadow copy may rely on the latest
committed version to generate return values.
Modeling this behavior, our lazy optimistic transactions
\PULL{} to retrieve the committed effects on a Proustian object
perform \APPLY{} rules to step forward but,
unlike the previous variants, do not perform \PUSH{} rules until it
has been determined (lazily) that the transaction can commit.

Consider an execution of transation $T$, during which a conflicting transaction,
$T'$, commits.
$T'$ replays its log on each Proustian object, updating
the object to a new committed version, possibly invalidating future $T$ operations: $T$'s
shadow copy may consult the underlying data structure
for return values and view the effects of $T'$.
In response, we surround execution of a Proustian operation $m_i$
with the relevant conflict abstraction operations $CA(m_i)$, as discussed
in the pseudocode above.
Together, these sets of \var{write}s and \var{read}s check whether
some other transaction $T'$ has committed a conflicting operation $n_j$.
During the commit of $T'$, the underlying STM will grant $T'$ exclusive
access to all \var{mem} locations accessed by $T'$, including the
regions of \var{mem} for references and for conflict abstraction locations
\anno{ $T'$ performs \PUSH{}($n_j$) for each operation $n_j$,
  \PUSH{}(read($x$))/\PUSH{}(write($x$)) for every accessed $x$,
  and then \CMT{} }.
The \var{write} operations above announce $m_i$ via the conflict
abstraction operations on \var{mem}. The \var{read} operations, if
they do not trigger an abort,
ensure that the transaction is working with a shadow copy
that has not been recently invalidated due to $T'$ committing a conflicting $n_j$
(whose conflict abstraction $CA(n_j)$ overlaps with $CA(m_i)$)
\anno{ Otherwise, $T$ does not perform \APPLY{}($m_i$) and instead
invokes \UNAPP{}($m_{i-1}$), etc in reverse order}.
  \end{proof}
\end{theorem}





The consequence of these careful algorithms is that, despite lazy conflict
detection, it is still impossible for a transaction to observe the
effects of another concurrent uncommitted transaction.



==> proust/opacitypess.tex <==
\section{Opacity}
\label{sec:opacity}
\emph{Opacity}~\cite{opacity} is a correctness condition (simplifying somewhat),
ensuring that committed transactions appear to have executed in a serial order,
and that aborted transactions observed consistent memory states at all times.
Modern STMs typically guarantee opacity.
\added{In this section we prove that transactional objects using conflict
  abstractions (Section~\ref{section:conflict}) and shadow copies (Section~\ref{section:shadow})
  satisfy opacity in three corners of the design space:
  (i) pessimistic transactional synchronization with eager updates,
  (ii) optimistic transactional synchronization with eager updates, and
  (iii) optimistic transactional synchronization with lazy updates.}
We begin with some background,
including the \emph{Push/Pull} formal semantic
model~\cite{KP:PLDI2015}, upon which we build our correctness
argument.


\paragraph{Preliminaries.}
A transaction $T$ consists of a sequence of data structure operations $m_1,m_2,...,m_n$.
For simplicity, we model state as a single array \var{mem} that has
two \emph{disjoint} regions:
$\var{mem}[\alpha,\beta,...]$ for conflict abstractions and
$\var{mem}[x,y,...]$ for shared variable references.
Both are managed by the same underlying STM.
Finally, for each operation $m_i$, the conflict abstraction
associated with $m_i$ is denoted $CA(m_i) \equiv \alpha_i^1,\alpha_i^2,\dots,\alpha_i^k$.

\paragraph{Background: Push/Pull.}
The Push/Pull model provides a general framework for aligning
transactional memory algorithms with
serializability/opacity arguments (via simulation relations)~\cite{KP:PLDI2015}.
The model has no concrete state but instead
consists of a single shared global log of operations,
as well as per-transactional local logs.
There are a few simple rules---named \PUSH{}, \PULL{}, etc.---that ferry (the names of)
ADT operations between these logs in ways that correspond to natural stages in a
transactional memory algorithm.
Different algorithms (pessimistic, optimistic, dependent transactions,
etc.)  combine these rules in different ways.
Here are some example stages.
A transaction perhaps begins by \PULL{}ing operations from the shared log
into its local log,
viewing effects that other transactions previously shared.
It then may take a step forward, appending a new operation $m$ to its local log via the \APPLY{}
rule.
Next, it may \PUSH{} this $m$ to the shared log, publishing this effect.
At this stage, the transaction may
not have committed (\eg\ when modeling boosting~\cite{HerlihyK2008},
commutative operations are \PUSH{}ed).
Meanwhile, the \PULL{} rule enables transactions to update
their local view with operations that are permanent (that is, they
correspond to committed transactions) or even to view the effects of
another uncommitted transaction (\eg, for eager conflict
detection~\cite{dstm} or dependent transactions~\cite{ut}).
One can also move in the reverse direction:
Push/Pull includes an \UNPULL{} rule which discards a
transaction's knowledge of an effect due to another thread, and an
\UNPUSH{} rule which removes a thread's operation from the shared
view, perhaps implemented as an inverse. The \UNAPP{} rule is useful
for rewinding a transaction's local state.  Finally, there is a simple
commit rule \CMT{} that, roughly, stipulates that all operations must
have been \PUSH{}ed and all \PULL{}ed operations must have been
committed.
(For lack of space, in the descriptions below, we will omit some detail
about how aborting is modeled with \UNPULL{} and \UNAPP{}.)


\paragraph{Pessimistic synchronization with eager updates.} 

\begin{theorem}\label{thm:pess} Pessimistic Proust is opaque.
  \begin{proof}(Sketch) 
   Based on~\cite{HerlihyK2008,KP:PLDI2015}. 
Conflict detection on Proustian
objects is done eagerly using abstract locks (as
in~\cite{HerlihyK2008}). In the Push/Pull model, this means that
transactions \APPLY{} locally, but do not \PUSH{} these effects
until they are sure the effects commute with all other
uncommitted operations that were \PUSH{}ed by other threads.
When another transaction commits, it is guaranteed not to conflict due to
the restriction that all \PUSH{}ed operations must commute.
It was shown~\cite{KP:PLDI2015} that this algorithm satisfies opacity.

Memory references $\var{mem}[x,y,...]$ may be
treated eagerly or lazily, depending on the underlying STM.
Ultimately, in either case, serializability is ensured because
all memory and Proustian object operations must be \PUSH{}ed
(which involves a conflict check) before \CMT{}.
With an eager STM, we model the STM's early knowledge of conflict
between memory references by \PUSH{}ing them to the shared log
immediately after they have been \APPLY{}ed locally.
Lazy memory references are modeled as transactions that
\PUSH{} Proustian object operations, but not \PUSH{}ing
memory operations until just before a commit. In this case, transactions
still cannot observe the effects of uncommitted transactions because
uncommitted \PUSH{}ed operations commute, and
reference variable have local-only views.
  \end{proof}
\end{theorem}


